When the LM misunderstood the human chuckled: Analyzing garden path effects in humans and language models

Modern Large Language Models (LLMs) have shown human-like abilities in many language tasks, sparking interest in comparing LLMs' and humans' language processing. In this paper, we conduct a detailed comparison of the two on a sentence comprehension task using garden-path constructions, which are notoriously challenging for humans. Based on psycholinguistic research, we formulate hypotheses on why garden-path sentences are hard, and test these hypotheses on human participants and a large suite of LLMs using comprehension questions. Our findings reveal that both LLMs and humans struggle with specific syntactic complexities, with some models showing high correlation with human comprehension. To complement our findings, we test LLM comprehension of garden-path constructions with paraphrasing and text-to-image generation tasks, and find that the results mirror the sentence comprehension question results, further validating our findings on LLM understanding of these constructions.

==> 01_intro.tex <==
\section{Introduction}

Humans are extremely skilled language comprehenders, correctly and effortlessly understanding the vast majority of sentences we meet. However, some syntactic structures pose challenges for accurate parsing. We tend to read these sentences more slowly and comprehend them less accurately. One such structure is the \emph{garden-path} sentence. These sentences are temporarily ambiguous, leading readers to misconstrue their meaning initially. Psycholinguistic research has shown that when asked reading comprehension questions about these sentences, humans tend to answer incorrectly. \emph{Cite Fereira} indicates that for garden-path sentences like \emph{While the man hunted the deer ran into the woods}, individuals overwhelmingly respond "Yes" to the question "Did the man hunt the deer?"

Large Language Models (LLMs), particularly transformer-based ones, serve as another example of proficient language comprehenders. These State-of-the-Art (SOTA) models have demonstrated performance that surpasses human capabilities across a range of tasks that demand diverse competencies, including reasoning, memory, and common sense understanding. Their ability to parse complex linguistic information and generate coherent, contextually appropriate responses highlights the advanced nature of these models in the domain of natural language processing.

Numerous studies have explored the capability of transformer-based Large Language Models (LLMs) to mimic human behavior in cognitive experiments across various domains, such as ethical decision-making and behavioral economics \emph{cite papers}. On a more granular level, several papers have spotlighted parallels in the way humans and LLMs process sentences. Some papers have compared the internal states of LLMs with neural activations in the human brain, uncovering significant correlations \emph{cite papers}. Other studies have examined the behavior of LLMs and humans when processing syntactic sentences, investigating whether both entities acquire similar syntactic structures \emph{cite paper}. With all these findings, one might be tempted to claim LLMs can serve as models of humans cognition.

We argue that showing that LLMs can overall mimic human behavior is not enough to make such claims. We claim that it is important as well to see if similar situations are challenging for both humans and LLMs. In the context of language processing, it means seeing if the same structures are challenging for accurate parsing for humans and LLMs.

Despite the growing interest in comparing humans and LLMs, there has been limited research specifically examining their similarities in reading comprehension tasks. Notably, the question of whether the same syntactic structures are complex for both humans and LLMs during reading comprehension remains under-explored. In typical reading comprehension tasks, participants—be they humans or LLMs—are presented with a sentence and subsequently asked to answer questions about it. \emph{Cite paper} replicated the experiments from \emph{cite paper} and discovered that LLMs also encounter difficulties with the specific type of garden-path sentences examined in the original study. Nonetheless, no thorough analysis has been conducted to determine what makes these sentences difficult for humans and if the same challenges apply to LLMs.

In this paper, we conduct an in-depth analysis of the sentence types discussed in \emph{cite Fereira}. Initially, we propose hypotheses regarding what makes these sentences challenging for human comprehension. We formulated four hypotheses and conducted experiments with human participants to test these theories. Our findings revealed that these sentences are difficult for several reasons, with three out of the four hypotheses being supported by the evidence. Subsequently, we applied the same experimental framework to LLMs to assess the similarity in behaviour between LLMs and humans in these tasks. Our results indicate that numerous LLMs exhibit significant behavioral similarities to humans in these experiments. Furthermore, we attempted to indirectly investigate what LLMs comprehend from these sentences, examining whether this understanding aligns with the errors LLMs make. We discovered that ...


==> 07_related_works.tex <==
\section{Related Work}

%\jb{Maybe this can have structure (a) past work on garden paths in humans (b) past work on humans vs. llms in general (c) past work on humans vs. LLMs on gardent paths?}

%Research comparing humans and LLMs language processing mechanism has been increasingly interesting with the recent progress in NLP.

%There has been two main strands of research in this area. The first investigates the similarity between the processes underlying human cognition and LLM processes by comparing the brain's to the LLM's internal activation. Some recent research has shown that the way \emph{LLMs} process sentences correlates with the way the brain processes these sentences. For example, \cite{fedorenko_brain_corr} showed that the most recent neural models' internal computations while processing a sentence can effectively predict brain activations (collected using fMRI and EEG) while reading the same sentence. Similarly, \cite{cacheteux-middle-layer} found that most LLM layers show some correlation with brain activation, with the middle layer showing the largest correlation. \citet{Ren2024DoLL} studied 23 different SOTA LLMs and found they all show some similarity with human brain activations, with the similarity to human activations being positively correlated with the LLM size, the pretraining data size and the alignment to humans.

%Other works compared LLMs with human behavior, rather than brain activity. For example, \citet{Rego2024LanguageMO} showed that LLMs outperform cloze predictability in modeling human sentence processing metrics like reading time and eye-gaze. \citet{Sun2024ComputationalSM} developed sentence-level metrics with multilingual LLMs and found they can predict reading time across a variety of languages. \citet{Li2024IncrementalCO} took 24 sentences from \cite{christianson2001} and measured reading comprehension on these sentences, showing that LLMs as well make the same misinterpretation as humans.

%\jb{use the paragraph environment to give this more structure.}

\paragraph{Garden path sentences} Garden path sentences hold a significant place in psycholinguistics, as they sparked the initial interest in processing difficulty. Early psycholinguistic research demonstrated that these sentences are read more slowly, specifically at the word or region where reanalysis is required \cite{gp3, gp2, gp1}. \citet{christianson2001} found that  comprehension is poorer for GP sentences of the type exemplified in (\ref{num:ex_gp}) compared to non-GP sentences as in (\ref{num:ex_ngp}). Specifically, the initial interpretation whereby the post-verbal NP is analyzed as the object of the first verb lingers, even while that same NP is also analyzed as the subject of the following verb (see also \citet{christianson2006}. Additionally, \citet{patson2009lingering} revealed that when participants were asked to paraphrase GP sentences, they often failed to perform full reanalysis and paraphrased the sentences inaccurately, e.g. ``The boy washed the dog and the dog barked'' for (\ref{num:ex_gp}). 

\paragraph{Comparing LLMs and humans} Research comparing LLM and human language processing mechanisms can be divided into two primary categories. The first category analyzes the correlation between brain and LLM activations while processing the same sentences, demonstrating that LLM activations significantly correlate with brain activities \cite{cacheteux-middle-layer, fedorenko_brain_corr, Ren2024DoLL}. The second category examines parallels in behavior, either by employing LLMs to predict human psycholinguistic metrics such as reading times \cite{Rego2024LanguageMO, Sun2024ComputationalSM} or learnability \cite{island_learnability}, or by highlighting that certain syntactic structures are challenging for both LLMs and humans \cite{neural-lms-subjects, wilcox-gpt2-abilities}.

\paragraph{LLMs and Garden Path sentences} Studies comparing LLMs and humans on garden path sentences fall into the second category described above. \citet{gp_reading_time} attempted to predict human reading times using LLM metrics and showed that LLM-based metrics vastly underestimate human reading times in various GP sentences. \citet{bert_gp} demonstrated that BERT representations are influenced by the GP effect. Finally, \citet{Li2024IncrementalCO} utilized object/subject GP sentences from \cite{christianson2001} to assess the sentence comprehension abilities of four different LLMs, revealing that these LLMs face similar difficulties with GP sentences to humans.

==> figures_dump.tex <==
\begin{figure*}[h!]
    \centering
    \scriptsize
    \includegraphics[height=20cm]{figures/per_category_spearman.pdf}
    \caption{Spearm rank correlation of categories per family}
    \label{fig:spearman_cats}
\end{figure*}

\begin{figure*}[h!]
    \centering
    \scriptsize
    \includegraphics[height=20cm]{figures/f1_value.pdf}
    \caption{F1 value of the different models on our significance metric}
    \label{fig:f1_value}
\end{figure*}

\begin{figure}[t]
    \centering
    \scriptsize
    \includegraphics[width=7cm, height=15cm]{figures/new_rank_correlation.pdf}
    \caption{Kendall Tau rank correlation between humans and different LLMs}
    \label{fig:kendall_tau}
\end{figure}

\begin{figure}[t!]
    \centering
    \includegraphics[width=8.0cm, height=6cm, trim={0.1cm 0.2cm 0.2cm 0.2cm}, clip]{figures/precision_recall.pdf}
    \caption{Precision and recall of the significance metric for different models}
    \label{fig:prec_recall}
    \vspace{-0.5cm}
\end{figure}
